Empirical relations for gravitational-wave asteroseismology of binary neutron star mergers

We construct new, multivariate empirical relations for measuring neutron star radii and tidal deformabilities from the dominant gravitational wave frequency in the post-merger phase of binary neutron star mergers. The relations determine neutron star radii and tidal deformabilities for specific neutron star masses with consistent accuracy and depend only on two observables: the post-merger peak frequency $f_{\rm peak}$ and the chirp mass $M_{\rm chirp}$. The former could be measured with good accuracy from gravitational waves emitted in the post-merger phase using next-generation detectors, whereas the latter is already obtained with good accuracy from the inspiral phase with present-day detectors. Our main data set consists of a gravitational wave catalogue obtained with CFC/SPH simulations. We also extract the $f_{\rm peak}$ frequency from the publicly available CoRe data set, obtained through grid-based GRHD simulations and find good agreement between the extracted frequencies of the two data sets. As a result, we can construct empirical relations for the combined data sets. Furthermore, we investigate empirical relations for two secondary peaks, $f_{2-0}$ and $f_{\rm spiral}$, and show that these relations are distinct in the whole parameter space, in agreement with a previously introduced spectral classification scheme. Finally, we show that the spectral classification scheme can be reproduced using machine-learning techniques.

==> eoschirp.tex <==
% This file was created by matplotlib2tikz v0.6.16.
\begin{tikzpicture}

\begin{axis}[
xlabel={Chirp Mass [$M_\odot$]},
ylabel={Equations of State},
xmin=1.001419140623998, xmax=1.684515339978,
ymin=0.2, ymax=13.6,
xtick={1,1.1,1.2,1.3,1.4,1.5,1.6,1.7},
xticklabels={1.0,1.1,1.2,1.3,1.4,1.5,1.6,1.7},
ytick={1,2,3,4,5,6,7,8,9,10,11,12,13},
yticklabels={tma,tm1,sly4,shen,sfhx,sfho,nl3,ls375,ls220,iuf,dd2,bhblp,apr},
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.21877078861457 9
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.23847157864814 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.56699101393302 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.10764597233269 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.4364084294386 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.04466067595535 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.47993595760341 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.30582584494419 10
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.26229831677938 10
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.27423051055392 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.30582584494419 12
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.42498173292546 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 10
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 3
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.47993595760341 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.27423051055392 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 13
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.30582584494419 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.26229831677938 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.23847157864814 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.10764597233269 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.21877078861457 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.3928809012738 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.04466067595535 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 10
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.30582584494419 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.3928809012738 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.04466067595535 10
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.27423051055392 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.56699101393302 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.20378556418443 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.34935337310899 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 4
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.35425875970748 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.35425875970748 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.4364084294386 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.21503604146428 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.04466067595535 9
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17427571650478 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.20378556418443 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.20378556418443 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.3928809012738 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.04466067595535 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.35425875970748 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.10764597233269 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17427571650478 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 12
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.23847157864814 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.65129543819752 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.21877078861457 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.42927392434415 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.21877078861457 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.13171573228496 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.65404607026264 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17427571650478 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.30582584494419 9
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.04466067595535 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.30582584494419 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.23847157864814 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.20378556418443 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.04466067595535 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.10764597233269 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.42927392434415 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.30582584494419 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.30582584494419 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 12
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.16651613497612 9
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.30582584494419 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 9
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.04466067595535 12
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.42927392434415 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17427571650478 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.21877078861457 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.3928809012738 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.10764597233269 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.3928809012738 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.04466067595535 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.04466067595535 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.13171573228496 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.17524326044977 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.38961378156017 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1.20378556418443 7
};


\path [draw=black, fill opacity=0] (axis cs:0,0.4)
--(axis cs:0,13.6);

\path [draw=black, fill opacity=0] (axis cs:1,0.4)
--(axis cs:1,13.6);

\path [draw=black, fill opacity=0] (axis cs:1.01419140623998,0)
--(axis cs:1.684515339978,0);
\end{axis}

\end{tikzpicture}

==> eosconf.tex <==
% This file was created by matplotlib2tikz v0.6.16.
\begin{tikzpicture}

\begin{axis}[
xlabel={Binary Mass Configuration [$M_\odot$]},
ylabel={Equations of State},
xmin=0, xmax=25,
ymin=0.4, ymax=13.6,
xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24},
xticklabels={1.2-1.2,1.2-1.35,1.2-1.5,1.2-1.6,1.2-1.8,1.3-1.3,1.3-1.4,1.3-1.5,1.35-1.35,1.35-1.5,1.35-1.8,1.35-2.0,1.4-1.4,1.45-1.45,1.5-1.5,1.5-1.7,1.5-1.8,1.55-1.55,1.6-1.6,1.65-1.65,1.7-1.7,1.8-1.8,1.8-2.0,1.9-1.9},
ytick={1,2,3,4,5,6,7,8,9,10,11,12,13},
yticklabels={tma,tm1,sly4,shen,sfhx,sfho,nl3,ls375,ls220,iuf,dd2,bhblp,apr},
xticklabel style = {rotate=90},
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black},
width=12cm,
height=8cm
]
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 1
25 1
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 2
25 2
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 3
25 3
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 4
25 4
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 5
25 5
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 6
25 6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 7
25 7
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 8
25 8
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 9
25 9
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 10
25 10
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 11
25 11
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 12
25 12
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
0 13
25 13
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
1 0
1 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
2 0
2 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
3 0
3 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
4 0
4 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
5 0
5 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
6 0
6 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
7 0
7 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
8 0
8 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
9 0
9 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
10 0
10 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
11 0
11 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
12 0
12 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
13 0
13 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
14 0
14 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
15 0
15 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
16 0
16 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
17 0
17 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
18 0
18 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
19 0
19 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
20 0
20 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
21 0
21 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
22 0
22 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
23 0
23 13.6
};
\addplot [very thin, white!50.196078431372548!black, dashed, forget plot]
table {%
24 0
24 13.6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
13 9
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
10 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
22 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
2 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
20 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
21 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
15 10
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
14 10
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
5 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
15 12
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
12 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 10
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 3
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
21 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
5 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 13
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
15 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
14 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
10 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
2 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
13 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
19 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 10
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
15 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
19 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1 10
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
5 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
22 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
4 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
18 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 4
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
11 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
11 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
20 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
8 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1 9
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
7 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
4 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
4 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
19 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
11 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
2 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
7 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 12
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
10 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
23 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
13 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
17 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
13 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
6 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
24 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
7 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
15 9
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
15 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
10 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
4 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
2 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 6
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
17 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
15 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
15 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 12
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
3 9
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
15 1
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 9
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1 12
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
17 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
7 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 5
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
13 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
19 8
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
2 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
19 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1 7
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
1 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
6 2
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
9 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
16 11
};
\addplot [semithick, black, mark=*, mark size=3, mark options={solid,fill=red}, forget plot]
table {%
4 7
};
\path [draw=black, fill opacity=0] (axis cs:0,0.4)
--(axis cs:0,13.6);

\path [draw=black, fill opacity=0] (axis cs:0,0)
--(axis cs:25,0);
\end{axis}

\end{tikzpicture}

==> firsthalf_freq_table.tex <==
\begin{table}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
\textbf{EoS} & \textbf{$\mathrm{f_{peak}}$} & \textbf{$\mathrm{f_{spiral}}$} & \textbf{$\mathrm{f_{2-0}}$} & \textbf{$\mathrm{M_{chirp}}$} & \textbf{$m_1$} & \textbf{$m_2$} & \textbf{$R_{1.4}$} & \textbf{$R_{1.6}$} & \textbf{$R_{1.8}$} \\ \hline
apr          & 3.46           & 2.68             & 2.33          & 1.18            & 1.35        & 1.35        & 11.34           & 11.27           & 11.14           \\ \hline
bhblp & 2.95 & 2.05 & nan & 1.31 & 1.5 & 1.5  & 13.14 & 13.12 & 12.95 \\ \hline
bhblp & 2.65 & nan & nan & 1.17 & 1.2 & 1.5 & 13.14 & 13.12 & 12.95 \\ \hline
bhblp & 2.61 & 1.87 & 1.55 & 1.18 & 1.35 & 1.35 & 13.14 & 13.12 & 12.95 \\ \hline
bhblp & 2.43 & 1.81 & nan & 1.04 & 1.2 & 1.2  & 13.14 & 13.12 & 12.95 \\ \hline
dd2          & 2.67           & 1.94             & 1.54          & 1.24            & 1.35        & 1.5         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 3.08           & -                & 2.18          & 1.44            & 1.65        & 1.65        & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.62           & -                & -             & 1.27            & 1.2         & 1.8         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.66           & 2.06             & 1.56          & 1.22            & 1.4         & 1.4         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.77           & 2.13             & 1.72          & 1.31            & 1.5         & 1.5         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.80           & -                & 1.72          & 1.35            & 1.35        & 1.8         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.50           & -                & -             & 1.20            & 1.2         & 1.6         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.96           & 2.32             & 1.97          & 1.39            & 1.6         & 1.6         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.55           & 1.86             & 1.41          & 1.17            & 1.3         & 1.4         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.54           & 1.95             & 1.29          & 1.13            & 1.3         & 1.3         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.61           & -                & -             & 1.17            & 1.2         & 1.5         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.94           & -                & 1.98          & 1.43            & 1.5         & 1.8         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.49           & 1.76             & 1.26          & 1.11            & 1.2         & 1.35        & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.41           & 1.80             & 1.20          & 1.04            & 1.2         & 1.2         & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.60           & 1.98             & 1.47          & 1.18            & 1.35        & 1.35        & 13.15           & 13.18           & 13.16           \\ \hline
dd2          & 2.90           & -                & 1.95          & 1.39            & 1.5         & 1.7         & 13.15           & 13.18           & 13.16           \\ \hline
ls220        & 3.06           & 2.54             & 2.07          & 1.22            & 1.4         & 1.4         & 12.56           & 12.36           & 12              \\ \hline
ls220        & 2.59           & 1.77             & 1.42          & 1.04            & 1.2         & 1.2         & 12.56           & 12.36           & 12              \\ \hline
ls220        & 3.43           & 2.59             & 2.32          & 1.31            & 1.5         & 1.5         & 12.56           & 12.36           & 12              \\ \hline
ls220        & 2.85           & -                & -             & 1.17            & 1.2         & 1.5         & 12.56           & 12.36           & 12              \\ \hline
ls220        & 2.87           & 2.18             & 1.72          & 1.18            & 1.35        & 1.35        & 12.56           & 12.36           & 12              \\ \hline
ls375        & 2.84           & -                & 1.91          & 1.48            & 1.7         & 1.7         & 13.57           & 13.67           & 13.72           \\ \hline
ls375        & 2.39           & 1.76             & 1.33          & 1.18            & 1.35        & 1.35        & 13.57           & 13.67           & 13.72           \\ \hline
ls375        & 3.07           & 2.42             & 2.11          & 1.57            & 1.8         & 1.8         & 13.57           & 13.67           & 13.72           \\ \hline
ls375        & 2.41           & -                & -             & 1.17            & 1.2         & 1.5         & 13.57           & 13.67           & 13.72           \\ \hline
ls375        & 2.23           & 1.65             & -             & 1.04            & 1.2         & 1.2         & 13.57           & 13.67           & 13.72           \\ \hline
ls375        & 2.56           & 1.83             & 1.50          & 1.31            & 1.5         & 1.5         & 13.57           & 13.67           & 13.72           \\ \hline
ls375        & 2.69           & 2.05             & 1.66          & 1.39            & 1.6         & 1.6         & 13.57           & 13.67           & 13.72           \\ \hline
nl3          & 2.58           & 1.81             & -             & 1.57            & 1.8         & 1.8         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.34           & -                & 1.38          & 1.42            & 1.35        & 2           & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.08           & -                & -             & 1.17            & 1.2         & 1.5         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.20           & 1.60             & -             & 1.24            & 1.35        & 1.5         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.19           & -                & -             & 1.27            & 1.2         & 1.8         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.15           & 1.60             & -             & 1.18            & 1.35        & 1.35        & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.27           & -                & 1.33          & 1.35            & 1.35        & 1.8         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.07           & 1.30             & -             & 1.11            & 1.2         & 1.35        & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.69           & 1.94             & -             & 1.65            & 1.8         & 2           & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.36           & -                & 1.45          & 1.43            & 1.5         & 1.8         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.79           & 2.10             & 1.83          & 1.65            & 1.9         & 1.9         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.33           & 1.60             & -             & 1.31            & 1.5         & 1.5         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.13           & 1.55             & -             & 1.17            & 1.3         & 1.4         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.37           & 1.79             & 1.39          & 1.39            & 1.6         & 1.6         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.04           & 1.47             & -             & 1.04            & 1.2         & 1.2         & 14.69           & 14.73           & 14.75           \\ \hline
nl3          & 2.07           & -                & -             & 1.20            & 1.2         & 1.6         & 14.69           & 14.73           & 14.75           \\ \hline
sfho         & 3.07           & -                & 1.85          & 1.11            & 1.2         & 1.35        & 11.81           & 11.68           & 11.43           \\ \hline
sfho         & 3.30           & -                & 2.15          & 1.20            & 1.2         & 1.6         & 11.81           & 11.68           & 11.43           \\ \hline
sfho         & 3.31           & -                & 2.34          & 1.22            & 1.3         & 1.5         & 11.81           & 11.68           & 11.43           \\ \hline
sfho         & 3.24           & -                & 2.21          & 1.17            & 1.3         & 1.4         & 11.81           & 11.68           & 11.43           \\ \hline
sfho         & 3.28           & 2.48             & 2.13          & 1.18            & 1.35        & 1.35        & 11.81           & 11.68           & 11.43           \\ \hline
sfho         & 3.39           & 2.51             & -             & 1.22            & 1.4         & 1.4         & 11.81           & 11.68           & 11.43           \\ \hline
\end{tabular}
\end{table}

==> secondhalf_freq_table.tex <==
\begin{table}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{eos} & \textbf{fpeak} & \textbf{fspiral} & \textbf{f2-0} & \textbf{Mchirp} & \textbf{m1} & \textbf{m2} & \textbf{R\_1.4} & \textbf{R\_1.6} & \textbf{R\_1.8} \\ \hline
  sfho         & 2.99           & 2.21             & 1.70          & 1.04            & 1.2         & 1.2         & 11.81           & 11.68           & 11.43           \\ \hline
sfho         & 3.13           & -                & 1.96          & 1.17            & 1.2         & 1.5         & 11.81           & 11.68           & 11.43           \\ \hline
sfhx         & 3.41           & 2.56             & 2.31          & 1.31            & 1.5         & 1.5         & 11.92           & 11.9            & 11.79           \\ \hline
sfhx         & 3.31           & 2.56             & 2.23          & 1.26            & 1.45        & 1.45        & 11.92           & 11.9            & 11.79           \\ \hline
sfhx         & 2.91           & 2.06             & 1.81          & 1.11            & 1.2         & 1.35        & 11.92           & 11.9            & 11.79           \\ \hline
sfhx         & 2.81           & 2.01             & 1.55          & 1.04            & 1.2         & 1.2         & 11.92           & 11.9            & 11.79           \\ \hline
sfhx         & 2.85           & -                & 1.86          & 1.17            & 1.2         & 1.5         & 11.92           & 11.9            & 11.79           \\ \hline
sfhx         & 3.06           & -                & -             & 1.20            & 1.2         & 1.6         & 11.92           & 11.9            & 11.79           \\ \hline
sfhx         & 3.20           & -                & 2.11          & 1.24            & 1.35        & 1.5         & 11.92           & 11.9            & 11.79           \\ \hline
sfhx         & 3.16           & 2.43             & 2.02          & 1.22            & 1.4         & 1.4         & 11.92           & 11.9            & 11.79           \\ \hline
sfhx         & 3.08           & 2.34             & 1.86          & 1.18            & 1.35        & 1.35        & 11.92           & 11.9            & 11.79           \\ \hline
shen         & 2.19           & -                & -             & 1.17            & 1.2         & 1.5         & -               & -               & -               \\ \hline
sly4         & 3.33           & 2.55             & 2.18          & 1.18            & 1.35        & 1.35        & 11.71           & 11.55           & 11.27           \\ \hline
tm1          & 2.23           & 1.43             & 1.16          & 1.17            & 1.2         & 1.5         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.90           & 2.11             & 1.61          & 1.48            & 1.7         & 1.7         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.44           & 1.64             & 1.32          & 1.27            & 1.2         & 1.8         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.61           & 2.01             & 1.67          & 1.39            & 1.6         & 1.6         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.56           & -                & 1.30          & 1.35            & 1.35        & 1.8         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.73           & 2.10             & 1.83          & 1.44            & 1.65        & 1.65        & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.25           & 1.65             & -             & 1.18            & 1.35        & 1.35        & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.25           & 1.54             & 1.23          & 1.17            & 1.3         & 1.4         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.12           & 1.52             & -             & 1.04            & 1.2         & 1.2         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.52           & 1.79             & 1.49          & 1.31            & 1.5         & 1.5         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.34           & 1.57             & 1.28          & 1.24            & 1.35        & 1.5         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.26           & -                & 1.18          & 1.20            & 1.2         & 1.6         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.17           & 1.46             & -             & 1.11            & 1.2         & 1.35        & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.74           & 1.87             & 1.71          & 1.43            & 1.5         & 1.8         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.33           & 1.73             & 1.20          & 1.22            & 1.4         & 1.4         & 14.38           & 14.26           & 14.06           \\ \hline
tm1          & 2.20           & 1.64             & -             & 1.13            & 1.3         & 1.3         & 14.38           & 14.26           & 14.06           \\ \hline
tma          & 2.15           & 1.64             & 1.15          & 1.04            & 1.2         & 1.2         & 13.72           & 13.57           & 13.24           \\ \hline
tma          & 2.97           & 2.18             & 1.63          & 1.39            & 1.6         & 1.6         & 13.72           & 13.57           & 13.24           \\ \hline
tma          & 2.75           & 2.13             & 1.84          & 1.35            & 1.55        & 1.55        & 13.72           & 13.57           & 13.24           \\ \hline
tma          & 2.33           & -                & 1.26          & 1.17            & 1.2         & 1.5         & 13.72           & 13.57           & 13.24           \\ \hline
tma          & 2.38           & 1.76             & 1.21          & 1.18            & 1.35        & 1.35        & 13.72           & 13.57           & 13.24           \\ \hline
tma          & 2.73           & 2.21             & 1.82          & 1.31            & 1.5         & 1.5         & 13.72           & 13.57           & 13.24           \\ \hline
\end{tabular}
\end{table}




==> tables/table2_f=2-0_e=0.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{2-0}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{RfM} and all masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{2-0}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   17.48   &   4.185   &  -9.647  &   -1.144   &   0.856   &  2.014   &  0.909   &  0.742  &  0.245  &  0.178  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   31.374   &   -19.386   &  -9.852  &   9.845   &   -0.763   &  2.753   &  0.918   &  0.646  &  0.218  &  0.167  \\ \hline
\textbf{$R_{1.4}$} &   17.73   &   3.279   &  -9.268  &   -0.923   &   1.214   &  1.713   &  0.935   &  0.636  &  0.207  &  0.154  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   30.105   &   -17.84   &  -9.364  &   8.874   &   -0.137   &  2.305   &  0.942   &  0.564  &  0.18  &  0.144  \\ \hline
\textbf{$R_{1.6}$} &   17.764   &   2.497   &  -8.797  &   -0.639   &   1.393   &  1.452   &  0.955   &  0.518  &  0.174  &  0.13  \\ \hline
\textbf{$R_{1.8}$} &   17.512   &   1.842   &  -8.211  &   -0.254   &   1.364   &  1.229   &  0.96   &  0.623  &  0.161  &  0.138  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   0.747   &   24.015   &  -7.446  &   -6.192   &   -2.413   &  3.136   &  0.83   &  0.569  &  0.184  &  0.17  \\ \hline
\end{tabular}
\label{f2-0_RfM_e0}
\end{table*}


==> tables/table2_f=2-0_e=0_fRM.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{2-0}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{fRM} and all masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{2-0}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   13.237   &   3.278   &  -1.894  &   -0.504   &   -0.107   &  0.066   &  0.785   &  0.383  &  0.105  &  0.081  \\ \hline
\textbf{$R_{1.4}$} &   11.549   &   3.76   &  -1.683  &   -0.26   &   -0.184   &  0.061   &  0.841   &  0.324  &  0.088  &  0.072  \\ \hline
\textbf{$R_{1.6}$} &   9.586   &   4.09   &  -1.427  &   0.048   &   -0.261   &  0.055   &  0.885   &  0.252  &  0.075  &  0.061  \\ \hline
\textbf{$R_{1.8}$} &   8.007   &   4.356   &  -1.241  &   0.558   &   -0.375   &  0.054   &  0.896   &  0.258  &  0.072  &  0.057  \\ \hline
\end{tabular}
\label{f2-0_fRM_e0}
\end{table*}


==> tables/table2_f=2-0_e=1.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{2-0}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{RfM} and only equal masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{2-0}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   13.015   &   7.143   &  -5.856  &   -1.883   &   0.059   &  1.049   &  0.873   &  0.679  &  0.272  &  0.183  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   29.638   &   -19.343   &  -7.525  &   9.087   &   0.521   &  1.454   &  0.871   &  0.595  &  0.259  &  0.157  \\ \hline
\textbf{$R_{1.4}$} &   14.129   &   5.692   &  -6.233  &   -1.602   &   0.71   &  0.881   &  0.912   &  0.573  &  0.227  &  0.155  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   28.249   &   -17.137   &  -7.399  &   7.988   &   0.9   &  1.22   &  0.912   &  0.506  &  0.205  &  0.147  \\ \hline
\textbf{$R_{1.6}$} &   15.271   &   4.123   &  -6.661  &   -1.188   &   1.23   &  0.783   &  0.942   &  0.465  &  0.186  &  0.13  \\ \hline
\textbf{$R_{1.8}$} &   16.527   &   2.287   &  -7.213  &   -0.562   &   1.618   &  0.778   &  0.951   &  0.626  &  0.165  &  0.146  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   34.725   &   -15.096   &  -15.795  &   4.743   &   2.745   &  3.623   &  0.779   &  0.597  &  0.176  &  0.18  \\ \hline
\end{tabular}
\label{f2-0_RfM_e1}
\end{table*}


==> tables/table2_f=2-0_e=1_fRM.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{2-0}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{fRM} and only equal masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{2-0}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   12.607   &   3.074   &  -1.791  &   -0.928   &   -0.012   &  0.058   &  0.718   &  0.366  &  0.114  &  0.077  \\ \hline
\textbf{$R_{1.4}$} &   10.859   &   3.586   &  -1.571  &   -0.706   &   -0.087   &  0.053   &  0.79   &  0.306  &  0.096  &  0.069  \\ \hline
\textbf{$R_{1.6}$} &   8.943   &   4.059   &  -1.332  &   -0.358   &   -0.182   &  0.048   &  0.849   &  0.229  &  0.08  &  0.061  \\ \hline
\textbf{$R_{1.8}$} &   7.797   &   4.773   &  -1.256  &   0.285   &   -0.357   &  0.055   &  0.86   &  0.269  &  0.075  &  0.061  \\ \hline
\end{tabular}
\label{f2-0_fRM_e1}
\end{table*}


==> tables/table2_f=peak_e=0.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{peak}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{RfM} and all masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{peak}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   44.776   &   -19.351   &  -14.253  &   4.19   &   3.615   &  1.52   &  0.929   &  0.731  &  0.225  &  0.156  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   56.906   &   -37.252   &  -15.701  &   11.756   &   3.638   &  1.83   &  0.951   &  0.526  &  0.19  &  0.134  \\ \hline
\textbf{$R_{1.4}$} &   43.865   &   -19.499   &  -13.296  &   4.392   &   3.463   &  1.338   &  0.952   &  0.621  &  0.182  &  0.135  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   55.809   &   -37.642   &  -14.473  &   12.15   &   3.41   &  1.609   &  0.968   &  0.493  &  0.154  &  0.109  \\ \hline
\textbf{$R_{1.6}$} &   43.796   &   -19.984   &  -12.921  &   4.674   &   3.371   &  1.26   &  0.969   &  0.526  &  0.144  &  0.117  \\ \hline
\textbf{$R_{1.8}$} &   45.02   &   -21.087   &  -13.382  &   5.111   &   3.385   &  1.323   &  0.972   &  0.647  &  0.141  &  0.124  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   28.796   &   -7.668   &  -6.631  &   0.516   &   3.478   &  -0.492   &  0.958   &  0.275  &  0.11  &  0.067  \\ \hline
\end{tabular}
\label{fpeak_RfM_e0}
\end{table*}


==> tables/table2_f=peak_e=0_fRM.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{peak}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{fRM} and all masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{peak}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   16.91   &   -1.896   &  -1.708  &   0.2   &   0.068   &  0.05   &  0.88   &  0.374  &  0.096  &  0.07  \\ \hline
\textbf{$R_{1.4}$} &   14.819   &   -1.474   &  -1.43  &   0.414   &   -0.0   &  0.043   &  0.916   &  0.337  &  0.078  &  0.062  \\ \hline
\textbf{$R_{1.6}$} &   12.696   &   -0.935   &  -1.17  &   0.713   &   -0.092   &  0.037   &  0.943   &  0.298  &  0.062  &  0.053  \\ \hline
\textbf{$R_{1.8}$} &   10.942   &   -0.369   &  -0.987  &   1.095   &   -0.201   &  0.036   &  0.948   &  0.247  &  0.06  &  0.05  \\ \hline
\end{tabular}
\label{fpeak_fRM_e0}
\end{table*}


==> tables/table2_f=peak_e=1.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{peak}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{RfM} and only equal masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{peak}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   41.63   &   -15.017   &  -13.692  &   2.903   &   3.089   &  1.525   &  0.919   &  0.69  &  0.232  &  0.151  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   52.201   &   -29.769   &  -15.398  &   8.918   &   3.333   &  1.832   &  0.945   &  0.52  &  0.191  &  0.131  \\ \hline
\textbf{$R_{1.4}$} &   40.891   &   -15.539   &  -12.71  &   3.235   &   2.967   &  1.333   &  0.949   &  0.578  &  0.181  &  0.129  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   51.229   &   -30.463   &  -14.143  &   9.46   &   3.09   &  1.612   &  0.966   &  0.412  &  0.147  &  0.108  \\ \hline
\textbf{$R_{1.6}$} &   41.316   &   -16.654   &  -12.458  &   3.722   &   2.936   &  1.269   &  0.969   &  0.462  &  0.139  &  0.108  \\ \hline
\textbf{$R_{1.8}$} &   43.685   &   -18.889   &  -13.352  &   4.505   &   3.075   &  1.397   &  0.969   &  0.654  &  0.136  &  0.128  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   33.802   &   -3.069   &  -15.522  &   -1.439   &   4.112   &  1.605   &  0.951   &  0.276  &  0.107  &  0.067  \\ \hline
\end{tabular}
\label{fpeak_RfM_e1}
\end{table*}


==> tables/table2_f=peak_e=1_fRM.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{peak}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{fRM} and only equal masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{peak}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   18.203   &   -1.505   &  -1.944  &   -0.16   &   0.107   &  0.057   &  0.893   &  0.257  &  0.092  &  0.06  \\ \hline
\textbf{$R_{1.4}$} &   16.013   &   -1.092   &  -1.649  &   0.104   &   0.031   &  0.049   &  0.93   &  0.227  &  0.073  &  0.052  \\ \hline
\textbf{$R_{1.6}$} &   13.822   &   -0.576   &  -1.375  &   0.479   &   -0.073   &  0.044   &  0.956   &  0.196  &  0.056  &  0.044  \\ \hline
\textbf{$R_{1.8}$} &   12.168   &   -0.049   &  -1.205  &   0.954   &   -0.197   &  0.044   &  0.953   &  0.215  &  0.055  &  0.048  \\ \hline
\end{tabular}
\label{fpeak_fRM_e1}
\end{table*}


==> tables/table2_f=spiral_e=0.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{spiral}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{RfM} and all masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{spiral}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   30.89   &   -10.914   &  -10.213  &   2.289   &   3.368   &  0.842   &  0.891   &  0.734  &  0.279  &  0.178  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   38.805   &   -20.695   &  -12.612  &   5.561   &   4.366   &  1.212   &  0.898   &  0.737  &  0.275  &  0.18  \\ \hline
\textbf{$R_{1.4}$} &   30.64   &   -11.693   &  -9.289  &   2.64   &   3.318   &  0.575   &  0.913   &  0.672  &  0.252  &  0.157  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   37.684   &   -20.594   &  -11.299  &   5.687   &   4.143   &  0.89   &  0.914   &  0.676  &  0.25  &  0.169  \\ \hline
\textbf{$R_{1.6}$} &   30.762   &   -12.647   &  -8.704  &   3.081   &   3.225   &  0.414   &  0.926   &  0.674  &  0.236  &  0.147  \\ \hline
\textbf{$R_{1.8}$} &   31.591   &   -14.039   &  -8.679  &   3.701   &   3.117   &  0.404   &  0.922   &  0.906  &  0.243  &  0.177  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   54.468   &   -38.851   &  -13.993  &   9.305   &   8.453   &  -0.614   &  0.921   &  0.34  &  0.138  &  0.082  \\ \hline
\end{tabular}
\label{fspiral_RfM_e0}
\end{table*}


==> tables/table2_f=spiral_e=0_fRM.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{spiral}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{fRM} and all masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{spiral}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   8.942   &   0.926   &  -0.926  &   -0.069   &   -0.061   &  0.028   &  0.773   &  0.438  &  0.109  &  0.079  \\ \hline
\textbf{$R_{1.4}$} &   7.356   &   1.321   &  -0.719  &   0.218   &   -0.141   &  0.024   &  0.814   &  0.383  &  0.1  &  0.07  \\ \hline
\textbf{$R_{1.6}$} &   6.107   &   1.666   &  -0.567  &   0.596   &   -0.234   &  0.022   &  0.845   &  0.316  &  0.092  &  0.063  \\ \hline
\textbf{$R_{1.8}$} &   5.846   &   1.75   &  -0.555  &   1.002   &   -0.316   &  0.026   &  0.846   &  0.27  &  0.089  &  0.066  \\ \hline
\end{tabular}
\label{fspiral_fRM_e0}
\end{table*}


==> tables/table2_f=spiral_e=1.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{spiral}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{RfM} and only equal masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{spiral}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   40.105   &   -17.154   &  -16.204  &   3.38   &   5.343   &  1.826   &  0.895   &  0.713  &  0.27  &  0.174  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   41.603   &   -14.538   &  -19.426  &   0.955   &   6.832   &  2.257   &  0.905   &  0.803  &  0.245  &  0.181  \\ \hline
\textbf{$R_{1.4}$} &   39.694   &   -17.542   &  -15.372  &   3.61   &   5.245   &  1.601   &  0.923   &  0.637  &  0.229  &  0.158  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   40.407   &   -14.521   &  -17.99  &   1.256   &   6.435   &  1.958   &  0.926   &  0.731  &  0.212  &  0.167  \\ \hline
\textbf{$R_{1.6}$} &   40.081   &   -18.359   &  -15.205  &   3.98   &   5.187   &  1.544   &  0.941   &  0.706  &  0.197  &  0.152  \\ \hline
\textbf{$R_{1.8}$} &   41.976   &   -20.13   &  -16.179  &   4.636   &   5.27   &  1.75   &  0.939   &  0.914  &  0.205  &  0.168  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   55.934   &   -37.162   &  -17.139  &   7.961   &   9.897   &  -0.382   &  0.951   &  0.212  &  0.117  &  0.05  \\ \hline
\end{tabular}
\label{fspiral_RfM_e1}
\end{table*}


==> tables/table2_f=spiral_e=1_fRM.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for $f_{\mathrm{spiral}}$ frequency as $f_{\mathrm{j}}$ in equation \ref{fRM} and only equal masses in mass configuration.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{spiral}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hline
\textbf{$R_{1.2}$} &   10.565   &   1.013   &  -1.185  &   -0.184   &   -0.052   &  0.038   &  0.788   &  0.422  &  0.097  &  0.081  \\ \hline
\textbf{$R_{1.4}$} &   8.687   &   1.398   &  -0.934  &   0.096   &   -0.13   &  0.032   &  0.835   &  0.37  &  0.083  &  0.075  \\ \hline
\textbf{$R_{1.6}$} &   7.019   &   1.756   &  -0.721  &   0.468   &   -0.222   &  0.028   &  0.872   &  0.306  &  0.074  &  0.065  \\ \hline
\textbf{$R_{1.8}$} &   6.264   &   1.929   &  -0.645  &   0.881   &   -0.311   &  0.03   &  0.877   &  0.286  &  0.075  &  0.061  \\ \hline
\end{tabular}
\label{fspiral_fRM_e1}
\end{table*}


==> tables/tables_combined-backup.tex <==
\begin{table*}[h]
\centering
\caption{Regression information for the empirical relation \ref{RfM}.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{$f_{\mathrm{peak}}$} & \textbf{$b_0$} & \textbf{$b_1$} & \textbf{$b_2$} & \textbf{$b_3$} &\textbf{$b_4$} &\textbf{$b_5$} & \textbf{$R^2$} & max res & mean res & $\sigma$ res \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|} 
\multicolumn{11}{| l |}{$f_{\mathrm{peak}}$ (equal masses)} \\ \hline
\textbf{$R_{1.2}$} &   41.63   &   -15.017   &  -13.692  &   2.903   &   3.089   &  1.525   &  0.919   &  0.69  &  0.232  &  0.151  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   52.201   &   -29.769   &  -15.398  &   8.918   &   3.333   &  1.832   &  0.945   &  0.52  &  0.191  &  0.131  \\ \hline
\textbf{$R_{1.4}$} &   40.891   &   -15.539   &  -12.71  &   3.235   &   2.967   &  1.333   &  0.949   &  0.578  &  0.181  &  0.129  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   51.229   &   -30.463   &  -14.143  &   9.46   &   3.09   &  1.612   &  0.966   &  0.412  &  0.147  &  0.108  \\ \hline
\textbf{$R_{1.6}$} &   41.316   &   -16.654   &  -12.458  &   3.722   &   2.936   &  1.269   &  0.969   &  0.462  &  0.139  &  0.108  \\ \hline
\textbf{$R_{1.8}$} &   43.685   &   -18.889   &  -13.352  &   4.505   &   3.075   &  1.397   &  0.969   &  0.654  &  0.136  &  0.128  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   33.802   &   -3.069   &  -15.522  &   -1.439   &   4.112   &  1.605   &  0.951   &  0.276  &  0.107  &  0.067  \\ 
\hhline{|=|=|=|=|=|=|=|=|=|=|=|} 
\multicolumn{11}{| l |}{$f_{\mathrm{peak}}$ (all masses)} \\ \hline
\textbf{$R_{1.2}$} &   44.776   &   -19.351   &  -14.253  &   4.19   &   3.615   &  1.52   &  0.929   &  0.731  &  0.225  &  0.156  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   56.906   &   -37.252   &  -15.701  &   11.756   &   3.638   &  1.83   &  0.951   &  0.526  &  0.19  &  0.134  \\ \hline
\textbf{$R_{1.4}$} &   43.865   &   -19.499   &  -13.296  &   4.392   &   3.463   &  1.338   &  0.952   &  0.621  &  0.182  &  0.135  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   55.809   &   -37.642   &  -14.473  &   12.15   &   3.41   &  1.609   &  0.968   &  0.493  &  0.154  &  0.109  \\ \hline
\textbf{$R_{1.6}$} &   43.796   &   -19.984   &  -12.921  &   4.674   &   3.371   &  1.26   &  0.969   &  0.526  &  0.144  &  0.117  \\ \hline
\textbf{$R_{1.8}$} &   45.02   &   -21.087   &  -13.382  &   5.111   &   3.385   &  1.323   &  0.972   &  0.647  &  0.141  &  0.124  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   28.796   &   -7.668   &  -6.631  &   0.516   &   3.478   &  -0.492   &  0.958   &  0.275  &  0.11  &  0.067  \\ 
\hhline{|=|=|=|=|=|=|=|=|=|=|=|} 
\multicolumn{11}{| l |}{$f_{\mathrm{2-0}}$ (equal masses)} \\ \hline
\textbf{$R_{1.2}^{sep}$} &   29.638   &   -19.343   &  -7.525  &   9.087   &   0.521   &  1.454   &  0.871   &  0.595  &  0.259  &  0.157  \\ \hline
\textbf{$R_{1.4}$} &   14.129   &   5.692   &  -6.233  &   -1.602   &   0.71   &  0.881   &  0.912   &  0.573  &  0.227  &  0.155  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   28.249   &   -17.137   &  -7.399  &   7.988   &   0.9   &  1.22   &  0.912   &  0.506  &  0.205  &  0.147  \\ \hline
\textbf{$R_{1.6}$} &   15.271   &   4.123   &  -6.661  &   -1.188   &   1.23   &  0.783   &  0.942   &  0.465  &  0.186  &  0.13  \\ \hline
\textbf{$R_{1.8}$} &   16.527   &   2.287   &  -7.213  &   -0.562   &   1.618   &  0.778   &  0.951   &  0.626  &  0.165  &  0.146  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   34.725   &   -15.096   &  -15.795  &   4.743   &   2.745   &  3.623   &  0.779   &  0.597  &  0.176  &  0.18 \\
\hhline{|=|=|=|=|=|=|=|=|=|=|=|} 
\multicolumn{11}{| l |}{$f_{\mathrm{2-0}}$ (all masses)} \\ \hline
\textbf{$R_{1.2}$} &   17.48   &   4.185   &  -9.647  &   -1.144   &   0.856   &  2.014   &  0.909   &  0.742  &  0.245  &  0.178  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   31.374   &   -19.386   &  -9.852  &   9.845   &   -0.763   &  2.753   &  0.918   &  0.646  &  0.218  &  0.167  \\ \hline
\textbf{$R_{1.4}$} &   17.73   &   3.279   &  -9.268  &   -0.923   &   1.214   &  1.713   &  0.935   &  0.636  &  0.207  &  0.154  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   30.105   &   -17.84   &  -9.364  &   8.874   &   -0.137   &  2.305   &  0.942   &  0.564  &  0.18  &  0.144  \\ \hline
\textbf{$R_{1.6}$} &   17.764   &   2.497   &  -8.797  &   -0.639   &   1.393   &  1.452   &  0.955   &  0.518  &  0.174  &  0.13  \\ \hline
\textbf{$R_{1.8}$} &   17.512   &   1.842   &  -8.211  &   -0.254   &   1.364   &  1.229   &  0.96   &  0.623  &  0.161  &  0.138  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   0.747   &   24.015   &  -7.446  &   -6.192   &   -2.413   &  3.136   &  0.83   &  0.569  &  0.184  &  0.17  
\\ 
\hhline{|=|=|=|=|=|=|=|=|=|=|=|} 
\multicolumn{11}{| l |}{$f_{\mathrm{spiral}}$ (equal masses)} \\ \hline
\textbf{$R_{1.2}$} &   40.105   &   -17.154   &  -16.204  &   3.38   &   5.343   &  1.826   &  0.895   &  0.713  &  0.27  &  0.174  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   41.603   &   -14.538   &  -19.426  &   0.955   &   6.832   &  2.257   &  0.905   &  0.803  &  0.245  &  0.181  \\ \hline
\textbf{$R_{1.4}$} &   39.694   &   -17.542   &  -15.372  &   3.61   &   5.245   &  1.601   &  0.923   &  0.637  &  0.229  &  0.158  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   40.407   &   -14.521   &  -17.99  &   1.256   &   6.435   &  1.958   &  0.926   &  0.731  &  0.212  &  0.167  \\ \hline
\textbf{$R_{1.6}$} &   40.081   &   -18.359   &  -15.205  &   3.98   &   5.187   &  1.544   &  0.941   &  0.706  &  0.197  &  0.152  \\ \hline
\textbf{$R_{1.8}$} &   41.976   &   -20.13   &  -16.179  &   4.636   &   5.27   &  1.75   &  0.939   &  0.914  &  0.205  &  0.168  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   55.934   &   -37.162   &  -17.139  &   7.961   &   9.897   &  -0.382   &  0.951   &  0.212  &  0.117  &  0.05  \\ \hline
\hhline{|=|=|=|=|=|=|=|=|=|=|=|} 
\multicolumn{11}{| l |}{$f_{\mathrm{spiral}}$ (all masses)} \\ \hline
\textbf{$R_{1.2}$} &   30.89   &   -10.914   &  -10.213  &   2.289   &   3.368   &  0.842   &  0.891   &  0.734  &  0.279  &  0.178  \\ \hline
\textbf{$R_{1.2}^{sep}$} &   38.805   &   -20.695   &  -12.612  &   5.561   &   4.366   &  1.212   &  0.898   &  0.737  &  0.275  &  0.18  \\ \hline
\textbf{$R_{1.4}$} &   30.64   &   -11.693   &  -9.289  &   2.64   &   3.318   &  0.575   &  0.913   &  0.672  &  0.252  &  0.157  \\ \hline
\textbf{$R_{1.4}^{sep}$} &   37.684   &   -20.594   &  -11.299  &   5.687   &   4.143   &  0.89   &  0.914   &  0.676  &  0.25  &  0.169  \\ \hline
\textbf{$R_{1.6}$} &   30.762   &   -12.647   &  -8.704  &   3.081   &   3.225   &  0.414   &  0.926   &  0.674  &  0.236  &  0.147  \\ \hline
\textbf{$R_{1.8}$} &   31.591   &   -14.039   &  -8.679  &   3.701   &   3.117   &  0.404   &  0.922   &  0.906  &  0.243  &  0.177  \\ \hline
\textbf{$R_{1.8}^{sep}$} &   54.468   &   -38.851   &  -13.993  &   9.305   &   8.453   &  -0.614   &  0.921   &  0.34  &  0.138  &  0.082  \\ \hline
\end{tabular}
\label{fpeak_RfM_e1}
\end{table*}





